Outfox: a Packet Format for a Layered Mixnet

Anonymous communication relies on encrypted packet formats that resist traffic analysis and ensure unlinkability. Sphinx, the current standard for mixnets, provides strong anonymity but relies on classical public-key cryptography, making it vulnerable to quantum attacks. In this paper, we present Outfox, a simplified variant of Sphinx tailored for mixnets with fixed-length routes and designed for post-quantum security. Outfox reduces both computational and communication costs. We formally define Outfox and prove its security in the Universal Composability (UC) framework. Our evaluation shows that Outfox retains strong anonymity guarantees while offering improved efficiency and adaptability to quantum-resistant cryptographic primitives.

==> WPES1introduction1PreviousWork.tex <==

\subsection{Related Work}
\label{wpes:sec:previouswork}

Anonymous packet formats have a long history of vulnerabilities due to the lack of formal security proofs. Early mixnets based on simple RSA encryption~\cite{DBLP:journals/cacm/Chaum81} were broken by active tagging attacks, where flipping a single bit allowed global adversaries to trace or drop packets~\cite{pfitzmann1990break}. Later designs like Minx addressed some flaws but relied on informal arguments, leaving them vulnerable to decryption attacks by an RSA bit oracle attack~\cite{shimshock2008breaking}. The Sphinx packet format~\cite{DBLP:conf/sp/DanezisG09} was introduced to resist such attacks, support anonymous replies, and provide formal security proofs. More recently, its security has been strengthened under the Universal Composability (UC) framework~\cite{scherer2024framework}.

Sphinx is a highly flexible packet format, unlike earlier mixnet packet designs limited to Chaumian cascade mixnets~\cite{moller2003provably}. Its versatility allows deployment across a wide range of mixnet architectures, including Chaumian cascades, layered topologies with interconnected mixes, and free-routing mixnets with variable-length paths~\cite{bohme2004pet}. As a result, Sphinx has become the default packet format for nearly all modern mixnet designs, including those requiring anonymous path setup~\cite{chen2015hornet, kate2010using}.
Although originally developed for anonymous communication, Sphinx has found use in diverse environments, such as Bitcoin's Lightning Network~\cite{kiayias2020composable}. 
Various attempts have been made to extend or modify Sphinx, including adapting it for multicast systems~\cite{hugenroth2021rollercoaster, schadt2024polysphinx}. However, some of these modifications have weakened its privacy properties. For example, proposals to incorporate authenticated encryption for the payload~\cite{beato2016improving} can cause packets to be dropped on tampering, rather than alerting the recipient as originally intended. Similarly, the EROR variant of Sphinx~\cite{klooss2024eror} revealed a subtle tagging attack if the first hop (gateway) and last hop (service provider) collude.

One limitation of Sphinx that remains unaddressed is its efficiency, particularly the heavy reliance on public key cryptography. When Sphinx was designed, "free-routing" mixnets like Mixminion~\cite{danezis2003mixminion}, where users or mixes could select arbitrary path lengths, were popular. As a result, Sphinx required complex padding mechanisms to ensure constant-size packet headers.
However, both theoretical and simulation studies have shown that mixnets with layered topologies and fixed-length routes provide stronger anonymity than those with variable-length paths~\cite{bohme2004pet, diaz2010impact, piotrowska2021studying}. This structure allows for significant simplification. In Outfox, we leverage the fixed route length to streamline packet construction and eliminate an entire key exchange. Unlike Sphinx, which maintains a constant-size header for all hops, Outfox allows the header to shrink as it progresses through the route. This per-layer reduction enables a simpler, more efficient design while preserving strong anonymity. In layered topologies, this approach is practical because each node knows its position in the route and the total route length is fixed, eliminating the need for uniform headers across all hops.

While Sphinx remains secure under standard computational assumptions, the emergence of quantum computing threatens its long-term viability. A sufficiently powerful quantum computer running Shor's algorithm could break the public key cryptography Sphinx relies on. Adapting Sphinx to use Key Encapsulation Mechanisms (KEMs) would enable post-quantum security by incorporating lattice-based schemes like ML-KEM~\cite{bos2018crystals} or hybrid KEMs that combine post-quantum and classical approaches, such as Xwing-KEM with Curve25519~\cite{connolly-cfrg-xwing-kem-02, bernstein2006curve25519}. The remaining symmetric components of Sphinx are comparatively resistant to quantum attacks and may only require parameter adjustments.
\ania{@Alfredo is there any other literature you want to include in this section?}

